Target Conditioned Sampling: Optimizing Data Selection for Multilingual Neural Machine Translation

To improve low-resource Neural Machine Translation (NMT) with multilingual corpora, training on the most related high-resource language only is often more effective than using all data available (Neubig and Hu, 2018). However, it is possible that an intelligent data selection strategy can further improve low-resource NMT with data from other auxiliary languages. In this paper, we seek to construct a sampling distribution over all multilingual data, so that it minimizes the training loss of the low-resource language. Based on this formulation, we propose an efficient algorithm, Target Conditioned Sampling (TCS), which first samples a target sentence, and then conditionally samples its source sentence. Experiments show that TCS brings significant gains of up to 2 BLEU on three of four languages we test, with minimal training overhead.

==> method.tex <==
\section{\label{sec:method} \dis}

\subsection{Settings}

\gn{Can we make the title something more descriptive than ``Settings''?}

Suppose our objective is to learn to translate from a source language $s$ into target language $t$ \gn{I made $s$ and $t$ lowercase, because we'll want to define a probability distribution over them later.}.
Let $f(x;\theta)$ be our translation model for a sentence $x$ in source language $s$, parameterized by $\theta$.
Given loss function $\mathcal{L}(f(x;\theta), y)$ \gn{This indicates that you are calculating translations first before calculating the loss function, which is not accuracte for MLE. Maybe re-write?}, 
%which measures how different $f(x;\theta)$ is to a sentence $y$ in the target, e.g. cross-entropy. Our objective is to minimize:
our objective is to minimize:
\begin{equation}
  \label{eqn:objective}
  \begin{aligned}
    \mathbb{E}_{x, y \sim P_s(X, Y)} [\mathcal{L}(f(x;\theta), y)]
  \end{aligned}
\end{equation}
where $P_s(X, Y)$ is the true distribution of $s$-$t$ parallel sentences over \emph{all} sentence pairs we may be asked to translate at test time.

Unfortunately, we do not have the true distribution $P(X, Y)$, so we must approximate it using the empirical distribution over training data
\begin{equation}
  \label{eqn:empirical}
  \hat{P}_s(X=x,Y=y) = \frac{c_s(x,y)}{\sum_{\tilde{x},\tilde{y}}c_s(\tilde{x},\tilde{y})}
\end{equation}
where $c_s(x,y)$ is the count of this sentence pair in our training dataset.
When we do not have much $s$-$t$ data, $\hat{P}_s(X,Y)$ is a poor approximation of $P_s(X,Y)$, and thus we are not able to learn effectively.
Within the monolingual context, there have been attempts at \emph{data selection} \cite{lots_of_papers_from_intro} and \emph{data augmentation} \cite{data_augmentation_for_low_resource_mt,switchout} that attempt to move $\hat{P}_s(X,Y)$ closer to $P_s(X,Y)$.

Another method for mitigating problems of insufficient training data in LRLs is multilingual training, where we have parallel data with multiple sources $s_1, s_2, \ldots, s_n$.
We assume $s_1$ is the language we want to translate, \textit{i.e.} $s=s_1$.
The simplest method to perform this training is to sample data unfiformly the concatenated training data of every language in the corpus:
\begin{equation}
  \label{eqn:concat}
  \hat{P}_{s_1,\ldots,s_n}(X=x,Y=y) = \frac{c_{s_1,\ldots,s_n}(x,y)}{\sum_{\tilde{x},\tilde{y}}c_{s_1,\ldots,s_n}(\tilde{x},\tilde{y})}.
\end{equation}
Another common strategy is language-weighted sampling \cite{johnson16multilingual,rapid_adapt_nmt}, where we define a probability over the source languages $P(S;\lambda)$, and first sample the language we want to use and then sample the data from that language's empirical distribution:
\begin{equation}
  \label{eqn:concat}
  P_{text{weight}}(X=x,Y=y;\lambda) = \sum_{i=1}^{n} \hat{P}_{s_i}(X=x,Y=y) P(S=s_i|\lambda)
\end{equation}
$P(S=s_i|\lambda)$ is hyperparameterized by mixture weights $\lambda$ that determine the proportion of data from each language that we use, \textit{i.e.} $P(S=s_i|\lambda) = \lambda_i$.
\gn{A comparison to a baseline that does this sort of up-sampling within the multilingual or HRL-LRL training paradigm would make the experiments stronger.}
The also-common method of selecting a single HRL $s_j$ similar to our target LRL $s_1$ \cite{multi_nmt_adapt} can be viewed as a special case of this framework, where $\lambda_i=0$ if $i \notin \{1,j\}$.

\subsection{Sampling Distribution Criterion}

Notably, all of these perform some sort of sampling over source and target sentences $x$, $y$, which are then fed into an arbitrary downstream translation system.
In the following, we will refer to this general sampling distribution as $Q(X,Y)$, with support over all sentences in $\{s_1,\ldots,s_n\}-t$.
We use $Q(X,Y)$ instead of $P(X,Y)$ to emphasize the fact that we can design this sampling distribution in an arbitrary way to achieve good training outcomes, specifically minimizing Eqn \ref{eqn:objective}.

But how can we construct a good $Q(X,Y)$?
One might initially consider selecting data that attempts to approximate $P_{s_1}(X,Y)$, as this is the data distribution over which we would like to achieve good translation results in the end.
However, there is an apparent problem with this: in most cases where $s_i \ne s_1$, if $P_{s_i}(X,Y) \ne 0$ then $P_{s_1}(X,Y) = 0$, and vice-versa.
This is simply because, by definition, sentences in different languages are almost always different -- if $s_1$ is Chinese and $s_i$ is French, an English sentence $y$ will rarely have the same translation in French and Chinese.

Thus, we must have another criterion.
In this paper, we argue that a good $Q(X,Y)$ distribution will have an expected loss
\begin{equation}
  \label{eqn:objective_q}
  \begin{aligned}
    \mathbb{E}_{x, y \sim Q(X, Y)} [\mathcal{L}(f(x;\theta), y)]
  \end{aligned}
\end{equation}
that is correlated with our objective Eqn \ref{eqn:objective} over the space of all $\theta$.
If this condition holds, training over data sampled from $Q(X,Y)$ can facilitate the learning of $\theta$.

\subsection{Constructing $Q(X,Y)$}

In the following, we propose \dis, which directly constructs $Q(X, Y)$ to more directly match the desired objective.
We first note that $Q(X, Y)$ should share some properties with $P(X, Y)$ to make Eqn \ref{eqn:objective_q} correlate well with Eqn \ref{eqn:objective}. 

First, $Q(X, Y)$ and $P(X, Y)$ should be \textbf{target invariant}.
That is, when marginalized to $Q(Y)$ and $P(Y)$, the probability distributions should match as closely as possible, as the target language $t$ is the same across all language pairs.
This property ensures that Eqn \ref{eqn:objective} and Eqn \ref{eqn:objective_q} are optimizing towards the same target $Y$ distribution.

\gn{There's no explanation of why this rank invariance property is desirable, so I got lost here. And also, as noted above if $x$ is not a sentence in $s_1$, $P_{s_1}(X=x|Y=y)$ will be zero most of the time, so the ranks will be tied, and meaningless most of the time. The only reason why multilingual NMT training works is because it is able to smooth over differences between the language when it does feature extraction on the encoder side. Defining a probability distribution over sentences is not very meaningful, so we need to think either in loss space (which sentences result in similar losses), or representation space (which sentences result in similar representations). I've stopped checking up to here, because we'll need to resolve this. I think you can argue that your similarity measures (vocab overlap and language model overlap) are likely to result in more similar representations or losses between the sentences. We can then validate that these measures are correlated in the experimental section.}
Second, $Q(X, Y)$ and $P(X, Y)$ should be \textbf{rank invariant}, which means that if we order data pairs in $S_i$-$t$ according to their probabilities in $Q$, their rank should be the same as if we order them by $P$.


Note the support of $Q$ is restricted to $S_i$-$t$, while the support of $P$ encompasses $S_i$-$t$ with very small probability mass \gn{}.
This property assigns higher weights to the loss of data pairs in $S_i$-$t$ with higher $P$ probability. Formally, we can define these properties as
\begin{itemize}
    \item Target Invariance:
    \begin{equation}
        \begin{aligned}
        \label{eqn:Q2}
        Q(Y) \approx P(Y)
        \end{aligned}
    \end{equation}
    \item Rank Invariance: 
    \begin{equation}
        \begin{aligned}
        \label{eqn:Q1}
        Q(X, Y) \propto P(X, Y)
        \end{aligned}
    \end{equation}
    Using Bayes rule, we can rewrite it as 
\begin{equation}
    \label{eqn:Q3}
    \begin{aligned}
    Q(X|y) = \frac{Q(X, Y)}{Q(y)} \propto \frac{P(X, Y)}{P(y)} = P(X|y)
    \end{aligned}
\end{equation}
\end{itemize}

Eqn \ref{eqn:Q2} and Eqn \ref{eqn:Q3} allow one to first sample y and then conditionally sample x during training.  



==> method_old.tex <==
\section{\label{sec:method}Method}
%\subsection{Settings}
Our objective is to learn to translate from a language $S$ into the target language $T$. Unfortunately, we do not have enough $S$-$T$ data, but instead, we have parallel data from multiple languages $S_1, S_2, ..., S_n$. In the following, we present \dis~(\disab), a probabilistic method that allows us to construct a sampling distribution over $S_i$-$T$ to facilitate the learning of translating from $S$ to $T$.

\subsection{\label{sec:importance_sampling}\dis}
Let $f_\theta(x)$ be our translation model for a sentence $x$ in the the language of interest $S$, where $\theta$ is the vector of parameters, and let $\mathcal{L}(x, y; \theta)$ be a loss function. Let $P(X, Y)$ models the joint distribution of $S$-$T$, with the domain over all parallel sequences of tokens, including the multilingual data $S_i$-$T$. 
%, which measures how different $f_\theta(x)$ is to a sentence $y$ in English, e.g. cross-entropy. 
Our objective is to minimize:
\begin{equation}
  \label{eqn:objective}
  \small
  \begin{aligned}
    \mathbb{E}_{x, y \sim P(X, Y)} [\mathcal{L}(x, y;\theta)]
  \end{aligned}
\end{equation}
As we do not know the distribution $P(X, Y)$, we use importance sampling, via a manually constructed distribution $Q(X, Y)$, to rewrite the objective in Eqn~\ref{eqn:objective} as follows
\begin{equation}
  \label{eqn:importance_1}
  \small
  \begin{aligned}
    &\mathbb{E}_{x, y \sim P(X, Y)} [\mathcal{L}(x, y; \theta)] = \sum_{x, y} P(x, y) \mathcal{L}(x, y; \theta) \\
    &= \sum_{x, y} Q(x, y) \cdot \frac{P(x, y)}{Q(x, y)} \cdot \mathcal{L}(x, y; \theta)
  \end{aligned}
\end{equation}
Using Bayes rule, we can rewrite Eqn~\ref{eqn:importance_1} as
\begin{equation}
  \label{eqn:importance_2}
  \small
  \begin{aligned}
    = \sum_{x, y} Q(x, y) \cdot \frac{P\left(x \middle| y \right) P(y)}{Q\left(x \middle| y \right) Q(y)} \cdot \mathcal{L}(x, y;\theta)
  \end{aligned}
\end{equation}
We now reverse an argument from~\citet{domain_adaptive_transfer_learning}, who assumes that the importance distribution $Q(X, Y)$ satisfies $P\left(X \middle| Y \right) \approx Q\left(X \middle| Y \right)$. Here, we restrict the choice of the importance distribution $Q$ to the ones that satisfy $P(Y) \approx Q(Y)$. This is a reasonable assumption, since with our definition of $P(X, Y)$, $P(Y)$ is just the target language model distribution, which many distributions can closely match. Now, thanks to the assumption that $P(y) \approx Q(y)$, we can rewrite Eqn~\ref{eqn:importance_2} as 
%~\zd{reverse the order of $\mathbb{E}_{y \sim Q(Y)}$ and $ \mathbb{E}_{x \sim P(X|y)}$?}
\begin{equation}
  \label{eqn:importance_3}
  \small
  \begin{aligned}
    &\approx \sum_{x, y} Q(x, y) \cdot \frac{P\left(x \middle| y \right)}{Q\left(x \middle| y \right)} \cdot \mathcal{L}(x, y; \theta) \\
    &=\sum_{x, y} Q(y) \cdot P\left(x \middle| y \right) \cdot \mathcal{L}(x, y; \theta) \\
    &=\mathbb{E}_{y \sim Q(Y)} \left[ \sum_{x} P\left(x \middle| y \right) \cdot \mathcal{L}(x, y; \theta) \right] \\
    &=\mathbb{E}_{y \sim Q(Y)} \mathbb{E}_{x \sim P(X|y)} \left[ \mathcal{L}(x, y;\theta) \right] 
  \end{aligned}
\end{equation}
\paragraph{Discussion.} 
The formulation in Eqn~\ref{eqn:importance_3} allows one to first sample $y$ and then conditionally sample $x$ during training.
%to perform stochastic updates,~\eg~Adam~\citep{adam}. 
Note that $P(X|y)$ is the back-translation probability distribution, so if one has access to a good estimate $\hat{P}(X|y)$, one can sample from it to have an \textit{unbiased estimation} of the training objective. This explains why \textit{sampling-based} back-translation outperforms beam-search based back-translation~\citep{back_translation_at_scale}.

\paragraph{Low Resource Solution.} In our setting of low-resource translation, we do not have enough $S$-$T$ parallel data to estimate $P(X|y)$ (otherwise, we can simply use that data to learn $f_\theta(x)$). We thus resort to a data augmentation policy $R_y(X)$ to sample the sentences $x$ for training. Thus, the training objective that we optimize is
\begin{equation}
  \label{eqn:importance_4}
  \small
  \begin{aligned}
    \mathbb{E}_{y \sim Q(Y)} \mathbb{E}_{x \sim R_y(X)} \left[ \mathcal{L}(x, y; \theta) \right]
  \end{aligned}
\end{equation}
Note that we do not apply importance sampling to sample $x$, as doing so necessitates estimating $\frac{P\left(x \middle| y \right)}{R_y(x)}$.
%, which is as difficult as estimating $P(X|y)$. 
Instead, we use $P(X|y)$ to guide the selection of $R_y(X)$, so that the importance weight $\frac{P\left(x \middle| y \right)}{R_y(x)} \approx 1$. Next, in Section~\ref{sec:choosing_distributions}, we discuss the choices of $Q(X, Y)$ and $R_y(X)$.

\subsection{\label{sec:choosing_distributions}Choosing the Sampling Distributions}
%Eqn~\ref{eqn:importance_4} allows us to define a training framework whenever we define the distributions $Q(X, Y)$ and $R_y(X)$. 
%In this section, we discuss the choices for the two distributions $Q(X, Y)$ and $R_y(X)$ in \disab.

\paragraph{Choosing $Q(X, Y)$.} In order to reduce Eqn~\ref{eqn:importance_2} to Eqn~\ref{eqn:importance_3}, we need the marginalization of $Q(X, Y)$ to $Q(Y)$ matches the distribution of $P(Y)$, which is the target language distribution. 

Specifically in our case, $P(Y)$ is simply the language model distribution over the target of $S$-$T$. We have parallel data from multiple languages $S_1, S_2, ..., S_n$, all into $T$, with the \textit{same domain} as $S$-$T$. Therefore, a uniform sample of an target sentence $y$ from the multilingual data can approximate $P(Y)$. We thus only need to sample $y$ uniformly from the union of all extra data. 
%In a more general case, where the multilingual data does not come from the same domain as $S$-$T$, we can estimate $P(Y)$ relatively easily using in-domain monolingual data. In this paper, we focus on a specific use case of our framework on the in-domain multilingual data, and leave the domain-general case as a future work.

\paragraph{Choosing $R_y(X)$.} There are two desiderata for $R_y(X)$. First, $R_y(X)$ should be diverse, so that we can better utilize data from the extra training languages. The diversity objective can be achieved by maximizing the entropy $\mathbb{H}[R_y(X)]$. Second, as discussed in Section~\ref{sec:importance_sampling}, $R_y(X)$ needs to be close to $P(X|y)$, in order to mitigate the bias in the objective in Eqn~\ref{eqn:importance_4}.

Conditioning on the same target $y$ and restricting the support of $P(X|y)$ (and hence of $R_y(X)$) to the sentences that translate into $y$ in at least one of $S_i$-$T$, $P(x|y)$ simply measures how likely $x$ is in $S$. We can quantify this property using a similarity measure $\text{sim}(x, S)$. Therefore, $R_y(X)$ should also maximize $\mathbb{E}_{x \sim R_y(X)}[\text{sim}(x, S)]$. Combining the two together, $R_y(X)$ should maximize:
\begin{equation}
  \small
  \begin{aligned}
     J(T) = \mathbb{E}_{x \sim R_y(x)} \left[ \text{sim}(x, S) \right] +  \tau \mathbb{H}\big[R_y(x)\big]
  \end{aligned}
\end{equation}
where $\tau$ is the temperature that controls the effect of diversity. The formulation here is similar to the data augmentation objective in~\citet{switchout}, which has the following analytical solution
\begin{align}
\small
  R^*_y(x) = \frac{\exp{(\text{sim}(x, L)/\tau)}}{\sum_{x'} \exp{(\text{sim}(x', L)/\tau)}}
\end{align}

\subsection{\label{subsec:alg}Algorithms}
 The formulation of $Q(X, Y)$ allows one to sample multilingual data with the following algorithm:
\setlist{nolistsep}
\begin{enumerate}[noitemsep]
    \item Select the target $y$ based on $Q(y)$. In our case we can simply use the uniform distribution. % $Q(y) = \frac{1}{|Y|}$
    \item Given the target size $y$, gather all data pairs $(x_i, y) \in U$ and calculate $\text{sim}(x_i, S)$
   \item Sample $(x_i, y)$ based on $R_y(X)$ 
\end{enumerate}
The algorithm requires calculating $R_y(X)$ repeatedly during training. To reduce this overhead, we propose two strategies for implementation: 1) \textbf{Stochastic}: compute $R_y(X)$ before training starts, and dynamically sample each minibatch using the precomputed $R_y(X)$; 2) \textbf{Deterministic}: compute $R_y(X)$ before training starts and select $x' = \argmax_{x} R_y(x)$ for training.
The deterministic method is equivalent to setting $\tau$, the degree of diversity in $R_y(X)$, to be 0.

\subsection{\label{subsec:sim}Similarity Measure}
%The algorithm in Section \ref{subsec:alg} requires a function $\text{sim}(L, x)$. that represents the similarity between the source sentence $x$ and $S$. 
In this section, we define two formulations of the similarity measure $\text{sim}(S, x)$, which is essential for constructing $R_y(X)$. 
\paragraph{Vocab Overlap} provides a crude measure of surface form similarity between two languages. It is efficient to calculate, and is often quite effective, especially for low-resource languages. 

First, the similarity between a sentence $x \in S_i$ and $S$ can be calculated at the document level:
\begin{align*}
  \small
    \text{sim}_{\text{vocab-doc}}(x, S) = \frac{| \text{vocab}_k(S) \cap \text{vocab}_k(S_i)|}{k}
\end{align*}
$\text{vocab}_k(\cdot)$ represents the top $k$ most frequent character $n$-grams in the training data of a language.

Second, this metric can be easily extended to the sentence level by replacing $\text{vocab}_k(L_i)$ to the set of character $n$-grams of all the words in the sentence $x$.
%\begin{align*}
%  \small
%    \text{sim}_{\text{vocab-sent}}(x, L) = \frac{| \text{vocab}_k(L) \cap \text{char-n}(x)|}{|\text{char-n}(x)|}
%\end{align*}
%where $\text{char-n}(\cdot)$ is the set of character $n$-grams of all the words in a sentence.
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}

\paragraph{Language Model} trained on $S$ can be used to calculate the probability that a data sequence belongs to $S$. Although it might not perform well if $S$ does not have enough training data, it can be easily used in the \disab~algorithms. The document-level metric is defined as: 
%A language level similarity between $x \in L_i$ and $L$ can be defined by the average character-level log likelihood for the entire training data of $L_i$. We take an exponential of the log likelihood so that the final metric is between 0 and 1:
\begin{align*}
  \small
    \text{sim}_{\text{LM-doc}}(x, S) = \text{exp}\left( \frac{\sum_{c_i \in S_i}\text{NLL}_{S} (c_i)}{|c_i \in S_i|}\right)
\end{align*}
where $\text{NLL}_L(\cdot)$ is negative log likelihood of a character-level LM trained on data from $S$.
Similarly, the corresponding sentence level metric is the LM probability over each sentence $x$. 
%\begin{align*}
%  \small
%    \text{sim}_{\text{LM-doc}}(x, L) = \text{exp}\left( \frac{\sum_{c \in x}\text{NLL}_{L} (c)}{|c \in x|}\right)
%\end{align*}
